Connectivity Games over Dynamic Networks

A game-theoretic model for the study of dynamic networks is analyzed. The model is motivated by communication networks that are subject to failure of nodes and where the restoration needs resources. The corresponding two-player game is played between "Destructor" (who can delete nodes) and "Constructor" (who can restore or even create nodes under certain conditions). We also include the feature of information flow by allowing Constructor to change labels of adjacent nodes. As objective for Constructor the network property to be connected is considered, either as a safety condition or as a reachability condition (in the latter case starting from a non-connected network). We show under which conditions the solvability of the corresponding games for Constructor is decidable, and in this case obtain upper and lower complexity bounds, as well as algorithms derived from winning strategies. Due to the asymmetry between the players, safety and reachability objectives are not dual to each other and are treated separately.

==> eptcsdata.tex <==
\providecommand{\firstpage}{131}
\providecommand{\publicationstatus}{Giovanna D'Agostino, Salvatore La Torre (Eds.):\\
Proceedings of the Second International Symposium on\\ 
``Games, Automata, Logics and Formal Verification'' (GandALF 2011)\\
EPTCS 54, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.54.10}{10.4204/EPTCS.54.10}}

